A Statistical Distance Derived From The Kolmogorov-Smirnov Test: specification, reference measures (benchmarks) and example uses

Statistical distances quantifies the difference between two statistical constructs. In this article, we describe reference values for a distance between samples derived from the Kolmogorov-Smirnov statistic $D_{F,F'}$. Each measure of the $D_{F,F'}$ is a measure of difference between two samples. This distance is normalized by the number of observations in each sample to yield the $c'=D_{F,F'}\sqrt{\frac{n n'}{n+n'}}$ statistic, for which high levels favor the rejection of the null hypothesis (that the samples are drawn from the same distribution). One great feature of $c'$ is that it inherits the robustness of $D_{F,F'}$ and is thus suitable for use in settings where the underlying distributions are not known. Benchmarks are obtained by comparing samples derived from standard distributions. The supplied example applications of the $c'$ statistic for the distinction of samples in real data enables further insights about the robustness and power of such statistical distance.

==> tables/tabNormNull.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ \\\hline
10.0 & 0.100 & 1.22 & 8 & 7 & 5 \\\hline
5.0 & 0.050 & 1.36 & 1 & 2 & 2 \\\hline
2.5 & 0.025 & 1.48 & 1 & 0 & 1 \\\hline
1.0 & 0.010 & 1.63 & 1 & 0 & 0 \\\hline
0.5 & 0.005 & 1.73 & 1 & 0 & 0 \\\hline
0.1 & 0.001 & 1.95 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for significance levels $\alpha$.
        The $c_1$ values were calculated using simulations of normal distributions with $\mu=0$ and $\sigma=1$.
        The $c_2$ values were calculated using simulations of normal distributions with $\mu=3$ and $\sigma=2$.
        The $c_3$ values were calculated using simulations of normal distributions with $\mu=6$ and $\sigma=3$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.7775$ and $\sigma(c_1)=0.2573$,
         $\mu(c_2)=0.7976$ and $\sigma(c_2)=0.2388$,
         $\mu(c_3)=0.7596$ and $\sigma(c_3)=0.2292$ .
        }
\end{center}
\end{table}

==> tables/tabNormNull_.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ \\\hline\hline
10.0 & {\bf 0.100} & 1.22 & 8 & 7 & 5 \\\hline
5.0 & {\bf 0.050} & 1.36 & 1 & 2 & 2 \\\hline
2.5 & {\bf 0.025} & 1.48 & 1 & 0 & 1 \\\hline
1.0 & {\bf 0.010} & 1.63 & 1 & 0 & 0 \\\hline
0.5 & {\bf 0.005} & 1.73 & 1 & 0 & 0 \\\hline
0.1 & {\bf 0.001} & 1.95 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for significance levels $\alpha$.
        The $c_1$ values were calculated using simulations of normal distributions with $\mu=0$ and $\sigma=1$.
        The $c_2$ values were calculated using simulations of normal distributions with $\mu=3$ and $\sigma=2$.
        The $c_3$ values were calculated using simulations of normal distributions with $\mu=6$ and $\sigma=3$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.7775$ and $\sigma(c_1)=0.2573$,
         $\mu(c_2)=0.7976$ and $\sigma(c_2)=0.2388$,
         $\mu(c_3)=0.7596$ and $\sigma(c_3)=0.2292$ .
        }
\end{center}
\end{table}

==> tables/tabPowerNull.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ & $|C_4(\alpha)|$ & $|C_5(\alpha)|$ \\\hline
10.0 & 0.100 & 1.22 & 13 & 10 & 10 & 10 & 9 \\\hline
5.0 & 0.050 & 1.36 & 8 & 3 & 7 & 5 & 7 \\\hline
2.5 & 0.025 & 1.48 & 5 & 2 & 3 & 2 & 2 \\\hline
1.0 & 0.010 & 1.63 & 3 & 0 & 1 & 1 & 1 \\\hline
0.5 & 0.005 & 1.73 & 1 & 0 & 0 & 1 & 1 \\\hline
0.1 & 0.001 & 1.95 & 0 & 0 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for critical values of $\alpha$.
        The $c_1$ values were calculated using simulations of power functions distributions with $a=0.3$.
        The $c_2$ values were calculated using simulations of power functions distributions with $a=1$.
        The $c_3$ values were calculated using simulations of power functions distributions with $a=2$.
        The $c_4$ values were calculated using simulations of power functions distributions with $a=3$.
        The $c_5$ values were calculated using simulations of power functions distributions with $a=4$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.8379$ and $\sigma(c_1)=0.3099$,
         $\mu(c_2)=0.8392$ and $\sigma(c_2)=0.2557$,
         $\mu(c_3)=0.8642$ and $\sigma(c_3)=0.2747$ .
         $\mu(c_4)=0.8383$ and $\sigma(c_4)=0.2724$ .
         $\mu(c_5)=0.7920$ and $\sigma(c_5)=0.2779$ .
        }
\end{center}
\end{table}

==> tables/tabPowerNull_.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ & $|C_4(\alpha)|$ & $|C_5(\alpha)|$ \\\hline\hline
10.0 & {\bf 0.100} & 1.22 & 13 & 10 & 10 & 10 & 9 \\\hline
5.0 & {\bf 0.050} & 1.36 & 8 & 3 & 7 & 5 & 7 \\\hline
2.5 & {\bf 0.025} & 1.48 & 5 & 2 & 3 & 2 & 2 \\\hline
1.0 & {\bf 0.010} & 1.63 & 3 & 0 & 1 & 1 & 1 \\\hline
0.5 & {\bf 0.005} & 1.73 & 1 & 0 & 0 & 1 & 1 \\\hline
0.1 & {\bf 0.001} & 1.95 & 0 & 0 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for critical values of $\alpha$.
        The $c_1$ values were calculated using simulations of power functions distributions with $a=0.3$.
        The $c_2$ values were calculated using simulations of power functions distributions with $a=1$.
        The $c_3$ values were calculated using simulations of power functions distributions with $a=2$.
        The $c_4$ values were calculated using simulations of power functions distributions with $a=3$.
        The $c_5$ values were calculated using simulations of power functions distributions with $a=4$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.8379$ and $\sigma(c_1)=0.3099$,
         $\mu(c_2)=0.8392$ and $\sigma(c_2)=0.2557$,
         $\mu(c_3)=0.8642$ and $\sigma(c_3)=0.2747$ .
         $\mu(c_4)=0.8383$ and $\sigma(c_4)=0.2724$ .
         $\mu(c_5)=0.7920$ and $\sigma(c_5)=0.2779$ .
        }
\end{center}
\end{table}

==> tables/tabUniformNull.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ \\\hline
10.0 & 0.100 & 1.22 & 9 & 9 & 4 \\\hline
5.0 & 0.050 & 1.36 & 5 & 4 & 0 \\\hline
2.5 & 0.025 & 1.48 & 2 & 1 & 0 \\\hline
1.0 & 0.010 & 1.63 & 0 & 0 & 0 \\\hline
0.5 & 0.005 & 1.73 & 0 & 0 & 0 \\\hline
0.1 & 0.001 & 1.95 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for critical values of $\alpha$.
        The $c_1$ values were calculated using simulations of uniform distributions within $[0,1)$.
        The $c_2$ values were calculated using simulations of uniform distributions within $[2,6)$.
        The $c_3$ values were calculated using simulations of uniform distributions with $\mu=4$ and $\sigma=10$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.8674$ and $\sigma(c_1)=0.2468$,
         $\mu(c_2)=0.8298$ and $\sigma(c_2)=0.2608$,
         $\mu(c_3)=0.7983$ and $\sigma(c_3)=0.2205$ .
        }
\end{center}
\end{table}

==> tables/tabUniformNull_.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ \\\hline\hline
10.0 & {\bf 0.100} & 1.22 & 9 & 9 & 4 \\\hline
5.0 & {\bf 0.050} & 1.36 & 5 & 4 & 0 \\\hline
2.5 & {\bf 0.025} & 1.48 & 2 & 1 & 0 \\\hline
1.0 & {\bf 0.010} & 1.63 & 0 & 0 & 0 \\\hline
0.5 & {\bf 0.005} & 1.73 & 0 & 0 & 0 \\\hline
0.1 & {\bf 0.001} & 1.95 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for critical values of $\alpha$.
        The $c_1$ values were calculated using simulations of uniform distributions within $[0,1)$.
        The $c_2$ values were calculated using simulations of uniform distributions within $[2,6)$.
        The $c_3$ values were calculated using simulations of uniform distributions with $\mu=4$ and $\sigma=10$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.8674$ and $\sigma(c_1)=0.2468$,
         $\mu(c_2)=0.8298$ and $\sigma(c_2)=0.2608$,
         $\mu(c_3)=0.7983$ and $\sigma(c_3)=0.2205$ .
        }
\end{center}
\end{table}

==> tables/tabWeibullNull.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{| l | c | c | c | c | c | c |}\hline
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ & $|C_4(\alpha)|$ \\\hline
10.0 & 0.100 & 1.22 & 0 & 9 & 5 & 9 \\\hline
5.0 & 0.050 & 1.36 & 0 & 1 & 3 & 3 \\\hline
2.5 & 0.025 & 1.48 & 0 & 0 & 1 & 1 \\\hline
1.0 & 0.010 & 1.63 & 0 & 0 & 1 & 0 \\\hline
0.5 & 0.005 & 1.73 & 0 & 0 & 1 & 0 \\\hline
0.1 & 0.001 & 1.95 & 0 & 0 & 0 & 0 \\\hline
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for critical values of $\alpha$.
        The $c_1$ values were calculated using simulations of 1-parameter Weibull distributions with $a=0.1$.
        The $c_2$ values were calculated using simulations of 1-parameter Weibull distributions with $a=2$.
        The $c_3$ values were calculated using simulations of 1-parameter Weibull distributions with $a=4$.
        Over all $N_c$ comparisons,
        The $N_o$ values of $c_4$ were calculated using simulations of
         1-parameter Weibull distributions with $a=6$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.1107$ and $\sigma(c_1)=0.0652$,
         $\mu(c_2)=0.8079$ and $\sigma(c_2)=0.2417$,
         $\mu(c_3)=0.7775$ and $\sigma(c_3)=0.2404$ .
         $\mu(c_4)=0.8209$ and $\sigma(c_4)=0.2389$ .
        }
\end{center}
\end{table}

==> tables/tabWeibullNull_.tex <==
\begin{table}[h!]
\begin{center}
\begin{tabular}{l | c | c || c | c | c | c}
$\alpha N_c$ & $\alpha$ & $c(\alpha)$ & $|C_1(\alpha)|$ & $|C_2(\alpha)|$ & $|C_3(\alpha)|$ & $|C_4(\alpha)|$ \\\hline
10.0 & {\bf 0.100} & 1.22 & 0 & 9 & 5 & 9 \\
5.0 & {\bf 0.050} & 1.36 & 0 & 1 & 3 & 3 \\\hline
2.5 & {\bf 0.025} & 1.48 & 0 & 0 & 1 & 1 \\
1.0 & {\bf 0.010} & 1.63 & 0 & 0 & 1 & 0 \\\hline
0.5 & {\bf 0.005} & 1.73 & 0 & 0 & 1 & 0 \\
0.1 & {\bf 0.001} & 1.95 & 0 & 0 & 0 & 0 \\
\end{tabular}
\caption{The theoretical maximum number $\alpha N_c$ of rejections
        of the null hypothesis for the critical value $\alpha$.
        The $c_1$ values were calculated using simulations of 1-parameter Weibull distributions with $a=0.1$.
        The $c_2$ values were calculated using simulations of 1-parameter Weibull distributions with $a=2$.
        The $c_3$ values were calculated using simulations of 1-parameter Weibull distributions with $a=4$.
        The $c_4$ values were calculated using simulations of 1-parameter Weibull distributions with $a=6$.
        Over all $N_c$ comparisons,
         $\mu(c_1)=0.1107$ and $\sigma(c_1)=0.0652$,
         $\mu(c_2)=0.8079$ and $\sigma(c_2)=0.2417$,
         $\mu(c_3)=0.7775$ and $\sigma(c_3)=0.2404$,
         $\mu(c_4)=0.8209$ and $\sigma(c_4)=0.2389$.
	}\label{tab:true}
\end{center}
\end{table}

